Camera Bias in a Fine Grained Classification Task

We show that correlations between the camera used to acquire an image and the class label of that image can be exploited by convolutional neural networks (CNN), resulting in a model that "cheats" at an image classification task by recognizing which camera took the image and inferring the class label from the camera. We show that models trained on a dataset with camera / label correlations do not generalize well to images in which those correlations are absent, nor to images from unencountered cameras. Furthermore, we investigate which visual features they are exploiting for camera recognition. Our experiments present evidence against the importance of global color statistics, lens deformation and chromatic aberration, and in favor of high frequency features, which may be introduced by image processing algorithms built into the cameras.

==> Sections/rebuttal.tex <==
\section{Author's Response}
\label{sec:rebuttal}

We thank all the reviewers for their insightful and constructive comments. 

\subsection{Reviewer 1}

\begin{itemize}
    \item \textit{``My only suggestion is to reconsider looking at the lens distortion experiment. Typically distortion is much more visible at the edges of the image, whereas the binary code data is mainly in the middle of the image.''} In addition to the backgrounds being mostly uniform, our images are all cropped from near the centre of a much larger image anyway. This means that even with a different pre-processing step such as Canny edges, which might show some peripheral features such as bottle edges in the cases where they are visible, there would be very little difference in the amount of lens distortion near the image borders.
\end{itemize}

\subsection{Reviewer 4}

\begin{itemize}
    \item \textit{``I would like to see at least a small mention on these (Algorithmic Transparency, Fairness, and Accountability) in the introduction and/or conclusion part''} {\color{orange} References to Algorithmic Transparency, Fairness and Accountability have been added in the introduction (paragraph 2 last sentence) and conclusion (paragraph 1 third sentence).}
    \item \textit{``...some of the images taken in the dataset have, at least in a part of them, something in the background. Do you think that this might affect you analysis? I would like to see an explanation to that in the dataset section of the paper.''} Although distractors are present in the background of many images, it should not affect the conclusions we can draw from out experiments unless these distractors correlate with manufacturer or camera type. We were aware of the camera bias issue at the time out dataset was acquired, and so care was taken to avoid this specific issue: four different people captured the images, and each photographed an equal number of bottles from each manufacturer using an equal number of each camera, to avoid any correlation between camera / manufacturer and photographer, since photographers may introduce their own systematic distractors e.g. by holding the bottles a different way. {\color{orange} This has been clarified in the dataset section (paragraph 2, sentences 3 - 6).}
\end{itemize}

\subsection{Reviewer 6}

\begin{itemize}
    \item \textit{``The authors claim that the CNNs identify camera types using high frequency features which are uniform throughout the image, but the adversarial attacks show rather localized perturbations, figure 5.''} We have used the term ``high frequencies'' somewhat loosely to refer to any spatially varying pattern that is detectable within a small window - {\color{magenta} this has been clarified in Section 4.D, sentence 2.}
    \item \textit{``They could show a heat map of all the perturbations on the entire dataset and show that it is uniform vs the the other model is localized around the text.''} Our claim that camera bias exploits high frequencies that are present throughout the image is supported by experiments classifying $32 \times 32$ image crops, particularly Figures \ref{fig:heatmap} and \ref{fig:singleimage_heatmap}. These figures show that camera classification is indeed possible from small image patches with no bias to any particular image region on average, although within individual images there are regions that cannot be classified accurately.
    \item \textit{``The claim that CNNs rely on the cameras types to classify seems a bit weak. To strengthen their argument, they could take the CNNs trained to classify current dataset and then use a different dataset with different objects but similarly biased with the same camera types and show that it is able to classify those images correctly.''} Training a CNN that cheats by exploiting camera bias and applying it to a new dataset with different objects but the same camera / label correlations would lend strength to our conclusions, but unfortunately we do not have access to the original cameras that captured our dataset. This is an issue because many of the potential sources of camera bias discussed in Section~\ref{sec:lit_review} produce fingerprints that are specific to individual cameras, not camera types. So a CNN that exploits camera / label correlations would not necessarily generalize to another camera biased dataset, even if the same camera types were used.
    \item \textit{``The training details were missing, e.g, loss function, how many layers of the used networks were retrained, any hyperparameters etc.''} {\color{magenta} Optimizer, weight decay, loss function and network pretraining details have been added to the first paragraph of Section 4.}
\end{itemize}

\subsection{Reviewer 7}

\begin{itemize}
    \item \textit{``the main problem of the paper is that it looks like a survey paper and not a conference paper''} We thank the reviewer for their criticism, however we would respectfully argue this is not a survey paper; we have reviewed relevant literature to identify potential sources of camera bias, and then importantly tested each hypothesis in turn using detailed experiments until we converged on built-in image processing as the most likely explanation. 
    \item \textit{``The authors just did some experiments to prove the authors' assumptions''} We thank the reviewer for their concern, but the original discovery that camera bias was the cause of poor generalization in our classification project took months of investigation; at no point did we assume this a priori. We believe the experiments in Section 4.2 demonstrate the role of camera bias quite adequately and we hope the reviewer agrees with the results of our experiments. 
    \item \textit{``It is lack of novelty in general.''} We would like to reaffirm that our contribution is novel as the problem of camera bias in deep learning has not been seriously investigated in any prior work to the best of our knowledge.
\end{itemize}

